Predictive Safety Guardrails Do Not Always Make LLM Agents Safer

Large language model agents increasingly take consequential actions in digital and physical environments, where safety risks may emerge only after multiple interaction steps. This has motivated world-model-driven predictive safety guardrails, which anticipate future consequences before execution. However, existing evaluations largely focus on end-to-end safety outcomes, leaving unclear whether safety gains arise from reliable prediction and faithful use of predicted risks. In this work, we systematically diagnose the prediction-to-action pipeline along three dimensions: how world-model predictions are integrated into decision making, whether the predictions themselves are reliable, and whether their content is faithfully used. Across seven policy models and two safety environments, we find that stronger prediction involvement does not yield monotonic safety gains and can reduce task completion while substantially increasing inference cost. We further find that world-model predictions remain insufficiently reliable, especially over longer horizons, where safety prediction degrades substantially relative to near-term forecasting. Finally, we find that safety gains can persist even under corrupted predictions, while locally verified predictions still leave subsequent safety violations, showing that predictive content is not faithfully incorporated into the decision process. Together, these findings expose a fundamental prediction-to-action gap in current predictive guardrails: producing more or seemingly accurate foresight is insufficient unless that foresight is both reliable and faithfully translated into safer decisions.

==> sections/statements.tex <==
\section*{Ethics Statement}
This work aims to support safer LLM agents by examining the reliability and limitations of predictive safety guardrails. Experiments use benchmark environments, recorded trajectories, and controlled interventions. The findings are intended to inform safety evaluation and mitigation, and should not be interpreted as guarantees of safety in real-world deployment.

\section*{Reproducibility Statement}
We provide the relevant code and supporting materials to facilitate reproducibility. The code is available at \href{https://github.com/REH502/rethinking-predictive-safety}{the project repository}. Detailed experimental settings, evaluation protocols, and metrics are described in Appendices A–E.

\section*{AI Use Statement}
Generative AI tools assisted with language polishing and literature research, manuscript drafting and translation, figure and LaTeX preparation, and the interpretation of results. The authors are responsible for verifying AI-assisted content and for the final manuscript and its claims.

